Implicit Neural Networks with Fourier-Feature Inputs for Free-breathing Cardiac MRI Reconstruction

Cardiac magnetic resonance imaging (MRI) requires reconstructing a real-time video of a beating heart from continuous highly under-sampled measurements. This task is challenging since the object to be reconstructed (the heart) is continuously changing during signal acquisition. In this paper, we propose a reconstruction approach based on representing the beating heart with an implicit neural network and fitting the network so that the representation of the heart is consistent with the measurements. The network in the form of a multi-layer perceptron with Fourier-feature inputs acts as an effective signal prior and enables adjusting the regularization strength in both the spatial and temporal dimensions of the signal. We study the proposed approach for 2D free-breathing cardiac real-time MRI in different operating regimes, i.e., for different image resolutions, slice thicknesses, and acquisition lengths. Our method achieves reconstruction quality on par with or slightly better than state-of-the-art untrained convolutional neural networks and superior image quality compared to a recent method that fits an implicit representation directly to Fourier-domain measurements. However, this comes at a relatively high computational cost. Our approach does not require any additional patient data or biosensors including electrocardiography, making it potentially applicable in a wide range of clinical scenarios.

==> figures/kfmlp/cava_v1/15/denoiser/sx.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.97)},
  anchor=north east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$s_{\text{x}} = s_{\text{y}}$},
xmin=3, xmax=30,
xtick style={color=black},
y grid style={darkgray176},
ylabel={SER},
ymin=7.6, ymax=8.8,
ytick style={color=black}
]

\addplot [semithick, steelblue31119180]
table {%
3 8.303
6 8.488
10 8.525
15 8.642
30 7.969
};

%\addplot [semithick, steelblue31119180]
%table {%
%3 1959
%6 1004
%10 484
%15 300
%30 272
%};

\end{axis}

\end{tikzpicture}


==> figures/kfmlp/cava_v1/20/denoiser/sx.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.97)},
  anchor=north east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$s_{\text{x}} = s_{\text{y}}$},
xmin=3, xmax=30,
xtick style={color=black},
y grid style={darkgray176},
ylabel={SER},
ymin=5.8, ymax=6.7,
ytick style={color=black}
]

\addplot [semithick, steelblue31119180]
table {%
3 0.012
6 6.08
10 6.511
15 6.47
30 6.42
};

%\addplot [semithick, steelblue31119180]
%table {%
%3 11
%6 1808
%10 1407
%15 601
%30 431
%};

\end{axis}

\end{tikzpicture}


==> figures/kfmlp/fully_sampled/fully_sampled_phantom_l2_sx_out_scale.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=0.501187233627272, xmax=1995262.31496888,
xmode=log,
ymode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000,100000,1000000,10000000,100000000},
y grid style={darkgray176},
ylabel={squared error},
ymin=200000.26875, ymax=10038260.60625,
ytick style={color=black},
]
\addplot [semithick, steelblue31119180]
table {%
1 4430380
10 3455135.25
100 3465778.25
1000 4227371
10000 3307665
100000 3310962.75
1000000 3315352.25
};
\addlegendentry{out scale=1.0}
\addplot [semithick, darkorange25512714]
table {%
1 2930029.25
10 1057450.25
100 778829.625
1000 1150012.125
10000 1199979.75
100000 1065951.375
1000000 1549457.625
};
\addlegendentry{out scale=10.0}
\addplot [semithick, forestgreen4416044]
table {%
1 2566103.5
10 551522.5
100 677624.1875
1000 656344.9375
10000 623610.0625
100000 690869.6875
1000000 964028.4375
};
\addlegendentry{out scale=30.0}
\addplot [semithick, crimson2143940]
table {%
1 2446715.75
10 449064.6875
100 409848.6875
1000 412874.78125
10000 440268.15625
100000 272767.875
1000000 410213.375
};
\addlegendentry{out scale=100.0}
\addplot [semithick, mediumpurple148103189]
table {%
1 3677196
10 1067446.625
100 1477420.125
1000 1497224.125
10000 1664781.625
100000 1564107.875
1000000 1686220.875
};
\addlegendentry{out scale=300.0}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/fully_sampled/l2_img.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=263.5,
xtick style={color=black},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=185.5,
ytick style={color=black},
ymajorticks=false,
xmajorticks=false,
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=263.5, ymin=185.5, ymax=-0.5] {figures/kfmlp/fully_sampled/export-001.png};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-13.15, xmax=276.15,
xtick style={color=black},
y grid style={darkgray176},
ymin=-44.2129933476853, ymax=931.70226779069,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 2.01519770417361
1 2.00548101302358
2 1.99751993324754
3 2.00376367618304
4 2.03185238972136
5 2.02401368122007
6 2.00153201907921
7 2.03790369524369
8 2.00706467119334
9 1.99635310646909
10 2.02383185281223
11 2.03217660974284
12 2.06109208624444
13 1.96909422807245
14 1.91760307717499
15 2.01415073822927
16 2.13483660819086
17 2.01878932039809
18 1.95556310490894
19 2.06787317627186
20 2.17076399841245
21 2.00483805282286
22 2.03799832550382
23 2.0622311715257
24 2.16095525459483
25 2.0125270186483
26 2.05958152093508
27 2.12028138523459
28 2.12362863592481
29 2.21293602426418
30 2.08811271434644
31 2.25878547016706
32 2.17673711294954
33 2.10978040331652
34 2.09189140623829
35 2.26496669009941
36 1.97171012895091
37 2.09136504224745
38 2.14214725071307
39 2.28537039020826
40 2.38003306337241
41 2.36440480845925
42 2.10546463866244
43 2.23489024251255
44 2.38273247242126
45 2.41469591024946
46 2.72514103900769
47 2.36226121922952
48 2.49529835274255
49 1.95606894038781
50 1.89542342684406
51 2.54332491968435
52 2.48954334865132
53 3.09004422931407
54 2.53279217051556
55 2.20766071333496
56 2.14053479073297
57 2.11400215523104
58 2.57316868943182
59 2.34733337617692
60 2.92052948337841
61 3.07936726894068
62 3.03107457401854
63 2.79914166849825
64 2.42827660787986
65 3.19731496675009
66 2.85844707088569
67 2.41167489390391
68 2.75103034757286
69 3.21061232237643
70 3.61152452946047
71 2.12260938670765
72 4.39290192582099
73 2.71992513051056
74 3.85681697320359
75 3.34294812344156
76 3.20170860507984
77 4.26143745001926
78 4.43494194440647
79 3.78321754029293
80 5.19173245196038
81 4.03328011411122
82 4.7687669998187
83 3.19701331809291
84 3.04663751972654
85 3.59439037328487
86 2.72169022399862
87 3.27915860741246
88 6.20734731635123
89 4.41054521553312
90 2.70712089433431
91 4.32943472635207
92 2.73000714974055
93 5.3571193195197
94 4.91540442379316
95 2.40896312780705
96 4.95132821398213
97 5.11811429069209
98 5.85351602871082
99 2.3437092523088
100 8.17861857953697
101 9.0925813656471
102 8.82637375095849
103 6.37979705736579
104 8.68569199121172
105 4.34497239734244
106 8.98459711526098
107 3.13424787649548
108 5.79053594242348
109 11.0168990563184
110 9.8598357914026
111 5.71966391977367
112 9.45367245478209
113 1.14956807083262
114 9.54052063974214
115 17.3913669279757
116 14.3509433378708
117 16.5723006135629
118 6.19052557130872
119 11.4354037189095
120 18.6057921031775
121 30.4933774650197
122 14.6346184327025
123 32.2123588769569
124 44.0497448283105
125 37.5218199575419
126 19.5554744366251
127 58.573028170724
128 135.384667092583
129 62.7117686849595
130 70.6563511740648
131 192.731187386969
132 887.342483193491
133 351.655264538562
134 42.6661529419972
135 73.8633963698585
136 120.446783498802
137 96.4509436353645
138 27.6086991793565
139 20.412360977721
140 45.0375355862058
141 31.6162647452543
142 31.0433562201072
143 20.087578589526
144 25.3287377020316
145 18.3226918240264
146 9.1244805149171
147 11.7977362743115
148 14.0343410941495
149 16.3105483692566
150 14.4677265224959
151 8.96550257282081
152 7.54946291191058
153 5.74087761331703
154 6.65594294695239
155 11.6633219309051
156 8.62129898923039
157 5.88262871823268
158 8.27926180587088
159 2.24996367981151
160 8.81296882381734
161 8.08257062218315
162 6.2419354219136
163 7.86542745362961
164 10.5995402814157
165 3.73972500500091
166 4.43912681051696
167 4.84068069483124
168 5.69000398841197
169 2.54008977013354
170 3.70964934374702
171 5.90659416593252
172 3.80810888658143
173 3.72739047097578
174 3.82721933079499
175 1.65568721219858
176 6.39134310979294
177 4.02011528949215
178 3.57590484887439
179 3.30524655126619
180 2.79877927296186
181 2.80079266243447
182 4.55492240409043
183 3.47250130457882
184 5.73202259926257
185 3.64533766070433
186 4.24493147232283
187 4.69874583437766
188 3.6535432734801
189 3.02194277136827
190 4.20388796881508
191 2.78750442001865
192 3.66339171114161
193 3.38901901113443
194 3.08755018988555
195 3.98140690002613
196 2.53669883837983
197 2.21859042995925
198 2.84020871950479
199 3.23924633916456
200 2.87304450274547
201 2.94814344530541
202 2.22438311235321
203 3.56000515312601
204 2.64476454902748
205 2.87630682650812
206 2.26960927058155
207 2.38257781070461
208 2.52481374728695
209 1.83873306305113
210 2.01138819353195
211 3.28558800692465
212 2.31870953074166
213 2.91347924763781
214 1.88270850104569
215 1.9539220565307
216 2.31873947064814
217 2.19569081331885
218 2.60067807871356
219 2.69065926582499
220 2.32893513687709
221 2.38692537678011
222 2.17928385401053
223 2.20701090540836
224 2.34223168448041
225 2.38451170298338
226 2.23888419328202
227 2.23520696133465
228 2.05583438196157
229 2.05739179476483
230 2.27211322036806
231 2.01897264777045
232 2.17242472230581
233 2.17839130696377
234 2.25523703042229
235 2.11815092108007
236 2.13007930846895
237 2.16633497738643
238 2.15816552514219
239 1.97749017668639
240 2.07598414697264
241 2.09231863989004
242 2.12349549987592
243 1.92484657870856
244 2.10772768426635
245 2.15663371867119
246 2.03064915526059
247 1.94991550502539
248 2.08492886874319
249 2.09561597825177
250 1.9643826962444
251 1.93152074858226
252 2.02632245445765
253 2.02216142061133
254 2.05945241713609
255 1.97352085141613
256 2.01762184336102
257 2.01273313220126
258 2.02441258724878
259 1.98759914412129
260 2.03630154356624
261 2.02425011915712
262 2.02007808837025
263 1.97742715734579
};
\addlegendentry{ground truth}

\addplot [semithick, darkorange25512714]
table {%
0 0.263197600841522
1 0.536082684993744
2 1.34745156764984
3 1.71324491500854
4 0.894543886184692
5 0.754875004291534
6 1.49771690368652
7 2.00710034370422
8 1.32767355442047
9 1.32645452022552
10 0.496648639440536
11 0.888965785503387
12 1.66091990470886
13 1.4943767786026
14 0.871534049510956
15 0.906158626079559
16 1.42348611354828
17 0.983927607536316
18 0.896063208580017
19 1.64277958869934
20 1.17246115207672
21 0.727953672409058
22 1.04460716247559
23 0.684354424476624
24 1.1145350933075
25 0.382239192724228
26 1.49359822273254
27 1.07598459720612
28 1.60293388366699
29 1.13346707820892
30 1.37230324745178
31 1.9150904417038
32 0.984577059745789
33 0.31421485543251
34 0.51085638999939
35 1.24554288387299
36 0.815446436405182
37 0.668321251869202
38 0.991028606891632
39 1.30585062503815
40 0.968040406703949
41 1.54204058647156
42 1.45769822597504
43 0.825659692287445
44 1.31767165660858
45 1.86973869800568
46 1.51461780071259
47 2.54907321929932
48 2.13803005218506
49 1.56108343601227
50 1.027960896492
51 2.1603798866272
52 2.39857387542725
53 1.78776288032532
54 1.36020231246948
55 2.45376634597778
56 1.15833258628845
57 0.304522156715393
58 1.45976746082306
59 1.59594678878784
60 2.30158948898315
61 1.97179448604584
62 2.16699266433716
63 2.99349856376648
64 0.421399593353271
65 2.81783485412598
66 0.815478563308716
67 2.06338858604431
68 1.95774006843567
69 2.99643969535828
70 3.07868576049805
71 0.937551736831665
72 3.40673780441284
73 1.59009599685669
74 1.71071398258209
75 3.22210812568665
76 2.5412962436676
77 1.37825930118561
78 2.59833717346191
79 4.12995862960815
80 4.83494424819946
81 3.49632525444031
82 4.66255664825439
83 2.16542220115662
84 2.70472097396851
85 2.35333228111267
86 3.09795260429382
87 2.39059066772461
88 6.34723329544067
89 3.70399165153503
90 2.18464827537537
91 4.11082553863525
92 2.47549533843994
93 3.42591571807861
94 3.30681991577148
95 1.21646571159363
96 5.33077144622803
97 4.96294260025024
98 5.76850938796997
99 2.32547950744629
100 6.98444557189941
101 7.62984752655029
102 8.95662307739258
103 7.48330116271973
104 8.61542701721191
105 4.1651725769043
106 9.15909671783447
107 1.98558700084686
108 5.74145221710205
109 10.3631954193115
110 6.65861558914185
111 4.99437570571899
112 9.54135990142822
113 1.27056038379669
114 9.95686531066895
115 17.6746158599854
116 13.9801197052002
117 16.9244575500488
118 7.35067653656006
119 11.6389942169189
120 18.6477642059326
121 30.5470886230469
122 14.5717763900757
123 32.2574691772461
124 44.0764503479004
125 37.4851112365723
126 19.6468563079834
127 58.6039276123047
128 135.401580810547
129 62.6300354003906
130 70.5776062011719
131 187.132217407227
132 665.28515625
133 314.030242919922
134 42.7073593139648
135 73.8768997192383
136 120.415565490723
137 96.4156036376953
138 27.6512985229492
139 20.4166259765625
140 45.0740814208984
141 31.4869022369385
142 31.1306018829346
143 20.1493587493896
144 25.3387298583984
145 18.3439197540283
146 9.1349401473999
147 12.3708906173706
148 13.8045873641968
149 16.2469959259033
150 14.4872121810913
151 7.62191343307495
152 7.64063787460327
153 1.99595475196838
154 8.18453407287598
155 10.9135665893555
156 8.21340465545654
157 4.710693359375
158 8.14013385772705
159 1.85081279277802
160 8.25224781036377
161 8.01152515411377
162 6.50934505462646
163 7.44844579696655
164 9.77867984771729
165 3.18669748306274
166 5.21975374221802
167 3.26806426048279
168 6.18358612060547
169 0.916215717792511
170 2.60504293441772
171 5.47928762435913
172 2.45738959312439
173 3.47050213813782
174 4.20196199417114
175 0.561653137207031
176 5.61379241943359
177 2.38989067077637
178 3.12954020500183
179 2.11282157897949
180 2.70931196212769
181 2.01685500144958
182 4.14109992980957
183 1.47330212593079
184 5.49163913726807
185 3.09210634231567
186 3.76463866233826
187 4.03270483016968
188 1.39558899402618
189 2.67731237411499
190 1.67001092433929
191 1.10401582717896
192 2.85554552078247
193 0.658508777618408
194 1.98156785964966
195 4.27106761932373
196 1.47197115421295
197 2.21453070640564
198 2.43133783340454
199 1.13445031642914
200 2.31476736068726
201 1.62717521190643
202 0.980634152889252
203 3.65276050567627
204 2.57806324958801
205 0.146791249513626
206 1.09576106071472
207 2.01153612136841
208 2.326247215271
209 0.409008413553238
210 0.695434749126434
211 2.33782362937927
212 1.70625352859497
213 2.60247468948364
214 0.372492998838425
215 0.349910229444504
216 0.153289675712585
217 1.24081599712372
218 2.30363249778748
219 2.11073136329651
220 1.06334686279297
221 1.29687702655792
222 1.23920929431915
223 0.558860838413239
224 0.477953970432281
225 0.869409739971161
226 1.34157991409302
227 2.25187849998474
228 0.730917811393738
229 0.862397611141205
230 0.836075007915497
231 2.10865569114685
232 0.567596912384033
233 0.70362263917923
234 1.27455806732178
235 0.944927930831909
236 0.953504800796509
237 1.99216842651367
238 1.46268701553345
239 0.621326088905334
240 1.15087330341339
241 1.31396663188934
242 0.782212495803833
243 0.727777540683746
244 1.12685036659241
245 1.74657094478607
246 1.12622117996216
247 0.569594264030457
248 0.392402499914169
249 0.776229500770569
250 0.489893913269043
251 0.276213318109512
252 1.28462982177734
253 0.913080990314484
254 1.57275891304016
255 0.93136864900589
256 0.784511387348175
257 1.86984431743622
258 1.6757025718689
259 0.753210365772247
260 1.0561261177063
261 0.567273259162903
262 0.84007853269577
263 1.14681363105774
};
\addlegendentry{reconstruction}
\end{groupplot}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/DMLP/vif_sx.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.97)},
  anchor=north east,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$s_{\text{x}} = s_{\text{y}}$},
xmin=0.00794328234724281, xmax=1.25892541179417,
xmode=log,
xtick style={color=black},
y grid style={darkgray176},
ylabel={VIF},
ymin=0.22902625054121, ymax=0.373193599283695,
ytick style={color=black}
]

\addplot [semithick, steelblue31119180]
table {%
0.01 0.300994694232941
0.05 0.342700988054276
0.15 0.366640537977219
0.25 0.328594475984573
0.5 0.325527429580688
1 0.235579311847687
};
\addlegendentry{$lr = \num{1e-4}$}

\addplot [semithick, darkorange25512714]
table {%
0.05 0.339
0.1 0.36443305015564
0.15 0.339
0.5 0.223252043128014
1 0.246002286672592
};
\addlegendentry{$lr = \num{2e-4}$}

\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/FMLP/num_epochs.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=2.38298470417284, xmax=377.67762353825,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
},
y grid style={darkgray176},
ylabel={number of epochs},
ymin=0, ymax=12000,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
3 10593.
10 6560.
30 1995.
100 4071.
300 920.
};
\addlegendentry{$\sout=3$}
\addplot [semithick, darkorange25512714]
table {%
3 3666.
10 5958.
30 1939.
100 4191.
300 4912.
};
\addlegendentry{$\sout=10$}
\addplot [semithick, forestgreen4416044]
table {%
3 5886.
10 6309.
30 2403.
100 2966.
300 2950.
};
\addlegendentry{$\sout=30$}
\addplot [semithick, crimson2143940]
table {%
3 4273.
10 8544.
30 2873.
100 5512.
300 4842.
};
\addlegendentry{$\sout=100$}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/FMLP/vif_highscore_img.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=263.5,
xtick style={color=black},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=185.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=263.5, ymin=185.5, ymax=-0.5] {figures/kfmlp/subsampled/cava_10/FMLP/max_vif_image_ksp-000.png};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-9.25, xmax=194.25,
xtick style={color=black},
y grid style={darkgray176},
ymin=-89.0780457735062, ymax=1916.8056835413,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 6.87649393081665
1 7.60814952850342
2 6.64363145828247
3 10.3267517089844
4 5.91972255706787
5 6.23961639404297
6 4.4856104850769
7 4.84228134155273
8 5.48408794403076
9 4.7126579284668
10 6.13846302032471
11 7.32925367355347
12 5.38639354705811
13 5.72814559936523
14 6.25653457641602
15 5.06428289413452
16 6.11209106445312
17 3.19178581237793
18 3.03520941734314
19 3.65348029136658
20 4.76472997665405
21 5.5057487487793
22 7.50622177124023
23 5.7865571975708
24 7.86141967773438
25 5.82888793945312
26 7.1959924697876
27 7.58825063705444
28 7.04579830169678
29 6.89784002304077
30 6.01046562194824
31 6.16748428344727
32 6.78987884521484
33 7.66204452514648
34 6.43331146240234
35 7.75121212005615
36 4.22318887710571
37 6.25335216522217
38 7.67983484268188
39 7.62315940856934
40 9.91602420806885
41 9.77304172515869
42 9.89446258544922
43 11.8082218170166
44 8.64552593231201
45 11.6792526245117
46 9.76381969451904
47 11.1372137069702
48 11.4164161682129
49 10.6277589797974
50 11.7373247146606
51 13.475923538208
52 13.8808898925781
53 16.145975112915
54 18.2088794708252
55 17.7924861907959
56 20.845796585083
57 21.2311229705811
58 24.4896049499512
59 31.8147678375244
60 35.509651184082
61 43.0377311706543
62 50.2208824157715
63 48.4189186096191
64 73.5141067504883
65 86.5012435913086
66 123.025634765625
67 167.056610107422
68 187.386291503906
69 265.993408203125
70 265.336181640625
71 267.234161376953
72 248.317749023438
73 190.927871704102
74 276.934020996094
75 279.332641601562
76 303.520416259766
77 410.562561035156
78 276.429504394531
79 177.550338745117
80 247.425903320312
81 218.372802734375
82 356.204193115234
83 510.083648681641
84 481.076263427734
85 603.910217285156
86 946.436828613281
87 1044.38598632812
88 1544.255859375
89 1825.62915039062
90 1701.58911132812
91 1769.79016113281
92 1592.71264648438
93 1119.18994140625
94 741.377990722656
95 272.817779541016
96 695.4033203125
97 417.077697753906
98 211.170516967773
99 291.985626220703
100 126.772041320801
101 98.6147232055664
102 261.712585449219
103 295.128204345703
104 335.240142822266
105 292.890686035156
106 347.413421630859
107 254.082565307617
108 308.376251220703
109 256.895355224609
110 284.447509765625
111 376.811798095703
112 277.708923339844
113 249.979293823242
114 128.193420410156
115 167.97834777832
116 95.9895095825195
117 121.470970153809
118 71.6048812866211
119 99.6151351928711
120 113.650695800781
121 172.624710083008
122 140.463562011719
123 194.685440063477
124 102.664596557617
125 174.319458007812
126 136.643768310547
127 139.647903442383
128 88.1758728027344
129 69.1450042724609
130 117.021903991699
131 92.8039779663086
132 101.161544799805
133 60.9396438598633
134 60.065845489502
135 25.4850215911865
136 56.7528190612793
137 52.5221405029297
138 52.3071403503418
139 49.9599838256836
140 36.2771987915039
141 51.4880867004395
142 32.0909805297852
143 47.4186897277832
144 16.0573692321777
145 34.3045501708984
146 29.7548999786377
147 32.3748588562012
148 18.8526000976562
149 7.23575735092163
150 39.4278106689453
151 28.4466781616211
152 62.313777923584
153 34.1513862609863
154 56.8915061950684
155 31.5521488189697
156 52.3342437744141
157 43.5888671875
158 42.6519470214844
159 40.2227210998535
160 26.7828426361084
161 15.7687206268311
162 11.3307085037231
163 14.9013214111328
164 17.221019744873
165 8.50733470916748
166 15.8362150192261
167 8.87003135681152
168 17.990514755249
169 21.3481178283691
170 26.2239589691162
171 39.2867660522461
172 39.6429481506348
173 34.1033592224121
174 30.0256385803223
175 17.4488868713379
176 5.26780986785889
177 2.78850913047791
178 10.997953414917
179 12.5497045516968
180 12.9794187545776
181 14.5913572311401
182 16.4473400115967
183 12.9568719863892
184 10.2419471740723
185 5.92170667648315
};
\addlegendentry{ground truth}

\addplot [semithick, darkorange25512714]
table {%
0 18.8291778564453
1 21.5725975036621
2 20.2567710876465
3 18.8642520904541
4 18.2482070922852
5 10.393424987793
6 11.696328163147
7 11.1286401748657
8 16.0426254272461
9 15.2037258148193
10 15.4822225570679
11 14.5897312164307
12 16.2103958129883
13 11.7279596328735
14 20.0500946044922
15 16.3918018341064
16 22.1497611999512
17 15.1872644424438
18 17.4279308319092
19 13.9563751220703
20 17.582368850708
21 12.6774349212646
22 15.1714744567871
23 6.61048555374146
24 5.63039636611938
25 15.2319927215576
26 21.4309711456299
27 24.9377059936523
28 23.4513492584229
29 19.9395008087158
30 28.745698928833
31 35.2975082397461
32 40.7620162963867
33 39.150577545166
34 39.6127014160156
35 29.9064750671387
36 36.460620880127
37 28.0395183563232
38 23.9400463104248
39 23.3972473144531
40 31.9624824523926
41 31.3214740753174
42 21.1525173187256
43 16.4932079315186
44 23.5117244720459
45 49.9952430725098
46 70.2562026977539
47 74.1553649902344
48 71.53759765625
49 84.8976593017578
50 89.9120712280273
51 116.122291564941
52 119.362991333008
53 129.455902099609
54 117.39266204834
55 96.8886260986328
56 93.1070327758789
57 82.8476104736328
58 128.96159362793
59 84.2050628662109
60 85.4496459960938
61 58.3304176330566
62 93.3976593017578
63 25.1241512298584
64 63.832576751709
65 132.384140014648
66 172.371017456055
67 276.234161376953
68 257.633575439453
69 299.859130859375
70 288.365936279297
71 266.211822509766
72 246.316635131836
73 188.00407409668
74 274.614379882812
75 280.373626708984
76 304.308837890625
77 410.944915771484
78 279.385192871094
79 182.71826171875
80 249.85791015625
81 218.633728027344
82 355.591247558594
83 511.252990722656
84 484.079010009766
85 606.263061523438
86 948.210021972656
87 1045.80322265625
88 1544.60913085938
89 1822.89294433594
90 1699.33276367188
91 1772.81799316406
92 1594.11315917969
93 1121.30688476562
94 743.060852050781
95 272.508270263672
96 697.563354492188
97 419.7958984375
98 211.20654296875
99 291.901000976562
100 124.85669708252
101 94.9741821289062
102 260.421752929688
103 297.623291015625
104 338.470733642578
105 291.626281738281
106 347.140960693359
107 257.359771728516
108 308.955200195312
109 256.066711425781
110 285.127868652344
111 376.073577880859
112 273.493865966797
113 245.706649780273
114 129.397109985352
115 168.72184753418
116 96.8987197875977
117 122.910774230957
118 69.1914520263672
119 101.530792236328
120 112.237075805664
121 168.130859375
122 139.15119934082
123 196.789749145508
124 105.527153015137
125 169.231063842773
126 135.873886108398
127 140.302947998047
128 85.1580429077148
129 66.9130935668945
130 114.91967010498
131 87.6737213134766
132 100.862396240234
133 57.9847526550293
134 60.043025970459
135 27.9880104064941
136 59.984489440918
137 53.2208023071289
138 49.1727180480957
139 46.2550048828125
140 35.214054107666
141 50.8716087341309
142 35.788703918457
143 51.0943336486816
144 20.4163722991943
145 35.1540756225586
146 22.1732063293457
147 27.6308460235596
148 18.7378425598145
149 6.06578588485718
150 37.8103981018066
151 27.9227848052979
152 57.7410659790039
153 27.7104930877686
154 57.3052062988281
155 32.567138671875
156 54.2162704467773
157 41.1949729919434
158 44.4989318847656
159 39.1459121704102
160 25.7938995361328
161 17.7454872131348
162 13.9341430664062
163 12.0561475753784
164 12.9796590805054
165 6.02618932723999
166 8.9348840713501
167 7.41554594039917
168 17.3215637207031
169 22.749210357666
170 28.5717620849609
171 34.6630859375
172 34.0729560852051
173 27.9739303588867
174 21.6055088043213
175 14.0279407501221
176 4.46151638031006
177 2.09848737716675
178 5.48176240921021
179 3.77551293373108
180 6.21916770935059
181 8.01917362213135
182 9.34049606323242
183 8.75112724304199
184 11.5248689651489
185 17.3136444091797
};
\addlegendentry{reconstruction}

\addplot [semithick, darkgray176, mark=*, mark size=1pt]
table {%
182 0
177 0
173 0
168 0
164 0
160 0
156 0
152 0
148 0
144 0
140 0
137 0
133 0
130 0
127 0
124 0
120 0
117 0
115 0
112 0
109 0
107 0
104 0
102 0
100 0
98 0
96 0
95 0
93 0
92 0
91 0
89 0
87 0
85 0
83 0
81 0
79 0
76 0
74 0
71 0
};

\addlegendentry{sampled indices}

\end{groupplot}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/FMLP/vif_out_scales_sx.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=2.38298470417284, xmax=377.67762353825,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
},
y grid style={darkgray176},
ylabel={vif},
ymin=0.0647335518151522, ymax=0.686326643452048,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
3 0.635571181774139
10 0.658072412014008
30 0.390595972537994
100 0.472526758909225
300 0.0929877832531929
};
\addlegendentry{$\sout=10$}
\addplot [semithick, darkorange25512714]
table {%
3 0.524220049381256
10 0.653647780418396
30 0.551273882389069
100 0.488500773906708
300 0.388038009405136
};
\addlegendentry{$\sout=30$}
\addplot [semithick, forestgreen4416044]
table {%
3 0.574656367301941
10 0.647886455059052
30 0.57947051525116
100 0.526847898960114
300 0.432672768831253
};
\addlegendentry{$\sout=100$}
\addplot [semithick, crimson2143940]
table {%
3 0.487570196390152
10 0.62572705745697
30 0.586582005023956
100 0.618435323238373
300 0.503654181957245
};
\addlegendentry{$\sout=300$}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/HDR_loss_no_sg/vif.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=0.794328234724281, xmax=125.892541179417,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000},
xticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
},
y grid style={darkgray176},
ylabel={vif},
ymin=0.00421488285064697, ymax=0.400487124919891,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
1 0.0304837878793478
3 0.0341214276850224
10 0.0496927872300148
30 0.0528463050723076
100 0.0502944812178612
};
\addlegendentry{10.0}
\addplot [semithick, darkorange25512714]
table {%
1 0.0222272574901581
3 0.032890759408474
10 0.140100330114365
30 0.135657653212547
100 0.154598250985146
};
\addlegendentry{100.0}
\addplot [semithick, forestgreen4416044]
table {%
1 0.123319156467915
3 0.136980980634689
10 0.141240835189819
30 0.15716552734375
100 0.165704637765884
};
\addlegendentry{1000.0}
\addplot [semithick, crimson2143940]
table {%
1 0.256650596857071
3 0.362478882074356
10 0.38247475028038
30 0.337017834186554
100 0.32043319940567
};
\addlegendentry{10000.0}

\addplot [semithick, steelblue31119180]
table {%
1 0.248235419392586
3 0.375165373086929
10 0.377361804246902
30 0.353533625602722
100 0.342695981264114
};
\addlegendentry{100000.0}
\addplot [semithick, darkorange25512714]
table {%
1 0.280250757932663
3 0.356238633394241
10 0.368575721979141
30 0.351119995117188
100 0.340776056051254
};
\addlegendentry{1000000.0}
\addplot [semithick, forestgreen4416044]
table {%
1 0.202419593930244
3 0.350973457098007
10 0.372126519680023
30 0.337388157844543
100 0.337915658950806
};
\addlegendentry{10000000.0}
\addplot [semithick, crimson2143940]
table {%
1 0.237961977720261
3 0.352277666330338
10 0.342157453298569
30 0.338494867086411
100 0.32220122218132
};
\addlegendentry{100000000.0}

\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/HDR_loss_no_sg/vif2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$\varepsilon$},
xmin=5, xmax=2000000,
xmode=log,
xtick style={color=black},
xtick={10,100,1000,10000,100000,1000000},
y grid style={darkgray176},
ylabel={vif},
ymin=0.00421488285064697, ymax=0.400487124919891,
ytick style={color=black}
]

\addplot [semithick, steelblue31119180]
table {%
10 0.0304837878793478
100 0.0222272574901581
1000 0.123319156467915
10000 0.256650596857071
100000 0.248235419392586
1000000 0.280250757932663
};
\addlegendentry{$\csx = 1$}

\addplot [semithick, darkorange25512714]
table {%
10 0.0341214276850224
100 0.032890759408474
1000 0.136980980634689
10000 0.362478882074356
100000 0.375165373086929
1000000 0.356238633394241
};
\addlegendentry{$\csx = 3$}

\addplot [semithick, forestgreen4416044]
table {%
10 0.0496927872300148
100 0.140100330114365
1000 0.141240835189819
10000 0.38247475028038
100000 0.377361804246902
1000000 0.368575721979141
};
\addlegendentry{$\csx = 10$}

\addplot [semithick, crimson2143940]
table {%
10 0.0528463050723076
100 0.135657653212547
1000 0.15716552734375
10000 0.337017834186554
100000 0.353533625602722
1000000 0.351119995117188
};
\addlegendentry{$\csx = 30$}

\addplot [semithick, darkgray176]
table {%
10 0.0502944812178612
100 0.154598250985146
1000 0.165704637765884
10000 0.32043319940567
100000 0.342695981264114
1000000 0.340776056051254
};
\addlegendentry{$\csx = 100$}

\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/HDR_loss_sg/vif.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$\varepsilon$},
xmin=79.4328234724281, xmax=1258925.41179417,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000,100000,1000000},
y grid style={darkgray176},
ylabel={vif},
ymin=0.230742333829403, ymax=0.400487124919891,
ytick style={color=black}
]
\addplot [semithick, crimson2143940]
table {%
100 0.287199139595032
1000 0.330228239297867
10000 0.238366186618805
100000 0.249283313751221
1000000 0.27410426735878
};
\addlegendentry{$\csx = 1$}
\addplot [semithick, steelblue31119180]
table {%
100 0.33083775639534
1000 0.378542840480804
10000 0.371804893016815
100000 0.368794918060303
1000000 0.362218379974365
};
\addlegendentry{$\csx = 3$}
\addplot [semithick, darkorange25512714]
table {%
100 0.342326104640961
1000 0.390843242406845
10000 0.380872368812561
100000 0.372866690158844
1000000 0.352810710668564
};
\addlegendentry{$\csx = 10$}
\addplot [semithick, forestgreen4416044]
table {%
100 0.34910786151886
1000 0.361526697874069
10000 0.353204339742661
100000 0.358869671821594
1000000 0.345859706401825
};
\addlegendentry{$\csx = 30$}
\addplot [semithick, mediumpurple148103189]
table {%
100 0.340133786201477
1000 0.350289672613144
10000 0.3448406457901
100000 0.344617515802383
1000000 0.339722514152527
};
\addlegendentry{$\csx = 100$}

\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/num_epochs2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.97)},
  anchor=north east,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=0.794328234724281, xmax=125892.541179417,
xmode=log,
xtick style={color=black},
xtick={1,10,100,1000,10000,100000,1000000,10000000},
y grid style={darkgray176},
ylabel={number of epochs},
ymin=0, ymax=10000,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
1 7537.
3 4507.
10 4959.
30 6034.
100 4161.
1000 2406
10000 5981
100000 7046
};
\addlegendentry{$\sout=30$}
\addplot [semithick, darkorange25512714]
table {%
1 4134.
3 3244.
10 3330.
30 2789.
100 1958.
1000 3075
10000 3053
100000 2467
};
\addlegendentry{$\sout=100$}
\addplot [semithick, forestgreen4416044]
table {%
1 5465.
3 2695.
10 2451.
30 1100.
100 1343.
1000 1331
10000 1223
100000 1924
};
\addlegendentry{$\sout=300$}
\addplot [semithick, crimson2143940]
table {%
1 3600.
3 4186.
10 2837.
30 1090.
100 1689.
1000 1270
10000 1542
100000 2293
};
\addlegendentry{$\sout=1000$}
\addplot [semithick, mediumpurple148103189]
table {%
1 7607.
3 9706.
10 4305.
30 2381.
100 1410.
1000 1730
10000 2391
100000 1754
};
\addlegendentry{$\sout=3000$}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/vif_highscore_img.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={
group size=2 by 1,
vertical sep=0.1cm,
    horizontal sep=2cm}]
\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=263.5,
xtick style={color=black},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=185.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=263.5, ymin=185.5, ymax=-0.5] {figures/kfmlp/subsampled/cava_10/max_vif_image_ksp-000.png};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-9.25, xmax=194.25,
xtick style={color=black},
y grid style={darkgray176},
ymin=-105.371425437927, ymax=2234.80807476044,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 6.87649393081665
1 7.60814952850342
2 6.64363145828247
3 10.3267517089844
4 5.91972255706787
5 6.23961639404297
6 4.4856104850769
7 4.84228134155273
8 5.48408794403076
9 4.7126579284668
10 6.13846302032471
11 7.32925367355347
12 5.38639354705811
13 5.72814559936523
14 6.25653457641602
15 5.06428289413452
16 6.11209106445312
17 3.19178581237793
18 3.03520941734314
19 3.65348029136658
20 4.76472997665405
21 5.5057487487793
22 7.50622177124023
23 5.7865571975708
24 7.86141967773438
25 5.82888793945312
26 7.1959924697876
27 7.58825063705444
28 7.04579830169678
29 6.89784002304077
30 6.01046562194824
31 6.16748428344727
32 6.78987884521484
33 7.66204452514648
34 6.43331146240234
35 7.75121212005615
36 4.22318887710571
37 6.25335216522217
38 7.67983484268188
39 7.62315940856934
40 9.91602420806885
41 9.77304172515869
42 9.89446258544922
43 11.8082218170166
44 8.64552593231201
45 11.6792526245117
46 9.76381969451904
47 11.1372137069702
48 11.4164161682129
49 10.6277589797974
50 11.7373247146606
51 13.475923538208
52 13.8808898925781
53 16.145975112915
54 18.2088794708252
55 17.7924861907959
56 20.845796585083
57 21.2311229705811
58 24.4896049499512
59 31.8147678375244
60 35.509651184082
61 43.0377311706543
62 50.2208824157715
63 48.4189186096191
64 73.5141067504883
65 86.5012435913086
66 123.025634765625
67 167.056610107422
68 187.386291503906
69 265.993408203125
70 265.336181640625
71 267.234161376953
72 248.317749023438
73 190.927871704102
74 276.934020996094
75 279.332641601562
76 303.520416259766
77 410.562561035156
78 276.429504394531
79 177.550338745117
80 247.425903320312
81 218.372802734375
82 356.204193115234
83 510.083648681641
84 481.076263427734
85 603.910217285156
86 946.436828613281
87 1044.38598632812
88 1544.255859375
89 1825.62915039062
90 1701.58911132812
91 1769.79016113281
92 1592.71264648438
93 1119.18994140625
94 741.377990722656
95 272.817779541016
96 695.4033203125
97 417.077697753906
98 211.170516967773
99 291.985626220703
100 126.772041320801
101 98.6147232055664
102 261.712585449219
103 295.128204345703
104 335.240142822266
105 292.890686035156
106 347.413421630859
107 254.082565307617
108 308.376251220703
109 256.895355224609
110 284.447509765625
111 376.811798095703
112 277.708923339844
113 249.979293823242
114 128.193420410156
115 167.97834777832
116 95.9895095825195
117 121.470970153809
118 71.6048812866211
119 99.6151351928711
120 113.650695800781
121 172.624710083008
122 140.463562011719
123 194.685440063477
124 102.664596557617
125 174.319458007812
126 136.643768310547
127 139.647903442383
128 88.1758728027344
129 69.1450042724609
130 117.021903991699
131 92.8039779663086
132 101.161544799805
133 60.9396438598633
134 60.065845489502
135 25.4850215911865
136 56.7528190612793
137 52.5221405029297
138 52.3071403503418
139 49.9599838256836
140 36.2771987915039
141 51.4880867004395
142 32.0909805297852
143 47.4186897277832
144 16.0573692321777
145 34.3045501708984
146 29.7548999786377
147 32.3748588562012
148 18.8526000976562
149 7.23575735092163
150 39.4278106689453
151 28.4466781616211
152 62.313777923584
153 34.1513862609863
154 56.8915061950684
155 31.5521488189697
156 52.3342437744141
157 43.5888671875
158 42.6519470214844
159 40.2227210998535
160 26.7828426361084
161 15.7687206268311
162 11.3307085037231
163 14.9013214111328
164 17.221019744873
165 8.50733470916748
166 15.8362150192261
167 8.87003135681152
168 17.990514755249
169 21.3481178283691
170 26.2239589691162
171 39.2867660522461
172 39.6429481506348
173 34.1033592224121
174 30.0256385803223
175 17.4488868713379
176 5.26780986785889
177 2.78850913047791
178 10.997953414917
179 12.5497045516968
180 12.9794187545776
181 14.5913572311401
182 16.4473400115967
183 12.9568719863892
184 10.2419471740723
185 5.92170667648315
};
\addlegendentry{ground truth}
\addplot [semithick, darkorange25512714]
table {%
0 29.7761898040771
1 26.8403434753418
2 23.4187602996826
3 24.699914932251
4 24.553689956665
5 26.0789375305176
6 33.1002235412598
7 43.3274955749512
8 43.638256072998
9 42.4750747680664
10 36.4300117492676
11 24.5373287200928
12 12.7134132385254
13 17.1357822418213
14 12.890308380127
15 15.6766481399536
16 13.2427062988281
17 17.9663715362549
18 25.1279487609863
19 34.7169761657715
20 37.2243499755859
21 40.727970123291
22 27.1204490661621
23 16.3829689025879
24 4.68693161010742
25 21.2306518554688
26 37.7423973083496
27 48.7339553833008
28 54.3265800476074
29 48.6541137695312
30 52.6229095458984
31 46.1015472412109
32 46.7836456298828
33 32.0097122192383
34 11.9898405075073
35 4.94763040542603
36 5.00637054443359
37 7.70061206817627
38 16.8280391693115
39 30.6283092498779
40 43.6543045043945
41 47.09423828125
42 47.0139541625977
43 40.9820785522461
44 31.9834270477295
45 22.4719142913818
46 2.35472822189331
47 22.2596187591553
48 37.7768020629883
49 43.3058052062988
50 49.2018814086914
51 54.4144821166992
52 52.2605133056641
53 44.0371589660645
54 41.5612373352051
55 34.2000274658203
56 36.4791069030762
57 33.322940826416
58 23.403678894043
59 19.56223487854
60 26.5222244262695
61 35.6574745178223
62 15.8774347305298
63 14.0434722900391
64 27.5224056243896
65 78.3979721069336
66 131.799102783203
67 209.885864257812
68 245.302597045898
69 223.02278137207
70 236.444244384766
71 264.574401855469
72 133.440734863281
73 75.6344223022461
74 274.551574707031
75 174.900131225586
76 303.494232177734
77 257.606262207031
78 39.1416282653809
79 175.165679931641
80 273.26611328125
81 211.200241088867
82 319.58984375
83 508.415008544922
84 434.416320800781
85 603.463012695312
86 793.431762695312
87 1042.91833496094
88 1421.10620117188
89 1823.47802734375
90 2128.43627929688
91 1769.87622070312
92 1595.65844726562
93 1118.15625
94 859.27099609375
95 272.958679199219
96 696.224792480469
97 342.088653564453
98 217.666290283203
99 137.098678588867
100 127.96752166748
101 410.139434814453
102 259.812042236328
103 346.620727539062
104 335.008911132812
105 150.151336669922
106 241.623260498047
107 254.397415161133
108 123.867553710938
109 259.345764160156
110 71.7765884399414
111 294.524749755859
112 273.986663818359
113 128.116516113281
114 206.292877197266
115 168.499038696289
116 27.2279472351074
117 123.203338623047
118 143.26448059082
119 48.0073661804199
120 122.747940063477
121 105.978340148926
122 93.4870300292969
123 119.013366699219
124 101.542366027832
125 91.4074783325195
126 16.5853900909424
127 144.642486572266
128 143.069976806641
129 118.948295593262
130 119.121559143066
131 160.228073120117
132 96.9437255859375
133 52.1182060241699
134 84.1076049804688
135 73.3681488037109
136 37.3268775939941
137 48.0264015197754
138 44.0164947509766
139 30.9129981994629
140 39.0489158630371
141 48.314510345459
142 30.428129196167
143 34.8086051940918
144 20.0615463256836
145 2.27593016624451
146 1.00037002563477
147 16.9210262298584
148 21.7653465270996
149 37.3677597045898
150 40.8688888549805
151 56.4364738464355
152 61.1339492797852
153 55.9621543884277
154 36.2873649597168
155 33.7316093444824
156 44.2628326416016
157 31.7153930664062
158 16.2154235839844
159 14.852331161499
160 24.4460754394531
161 12.6947193145752
162 14.4735956192017
163 16.847282409668
164 6.21123027801514
165 4.26782894134521
166 11.7824487686157
167 14.8349494934082
168 22.3755226135254
169 25.2535934448242
170 9.45724296569824
171 3.47003650665283
172 21.1428451538086
173 29.2109203338623
174 22.3942470550537
175 11.6020936965942
176 10.8610830307007
177 2.57265996932983
178 8.98286628723145
179 17.4323387145996
180 16.0253620147705
181 11.2323942184448
182 10.0157165527344
183 18.5008182525635
184 22.6775379180908
185 22.3151683807373
};
\addlegendentry{reconstruction}


\addplot [semithick, darkgray176, mark=*, mark size=1pt]
table {%
182 0
177 0
173 0
168 0
164 0
160 0
156 0
152 0
148 0
144 0
140 0
137 0
133 0
130 0
127 0
124 0
120 0
117 0
115 0
112 0
109 0
107 0
104 0
102 0
100 0
98 0
96 0
95 0
93 0
92 0
91 0
89 0
87 0
85 0
83 0
81 0
79 0
76 0
74 0
71 0
};

\addlegendentry{sampled indices}

\end{groupplot}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/vif_out_scales_sx.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=0.794328234724281, xmax=125892.541179417,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000,100000,1000000,10000000},
y grid style={darkgray176},
ylabel={vif},
ymin=0.253627194464207, ymax=0.380968110263348,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
1 0.297185719013214
3 0.287829875946045
10 0.325426697731018
30 0.340947091579437
100 0.315348893404007
1000 0.262865126132965
10000 0.331408947706223
100000 0.333941161632538
};
\addlegendentry{$\sout=30$}
\addplot [semithick, darkorange25512714]
table {%
1 0.279084116220474
3 0.341181099414825
10 0.351213216781616
30 0.343490421772003
100 0.314677864313126
1000 0.339577615261078
10000 0.329541891813278
100000 0.329014420509338
};
\addlegendentry{$\sout=100$}
\addplot [semithick, forestgreen4416044]
table {%
1 0.278837561607361
3 0.34683620929718
10 0.360887914896011
30 0.33306086063385
100 0.337219834327698
1000 0.333898425102234
10000 0.333896726369858
100000 0.336101144552231
};
\addlegendentry{$\sout=300$}
\addplot [semithick, crimson2143940]
table {%
1 0.259415417909622
3 0.352395474910736
10 0.372363120317459
30 0.352717041969299
100 0.342513650655746
1000 0.340898305177689
10000 0.342529624700546
100000 0.335768282413483
};
\addlegendentry{$\sout=1000$}
\addplot [semithick, mediumpurple148103189]
table {%
1 0.271917253732681
3 0.375179886817932
10 0.370100736618042
30 0.350876152515411
100 0.329820036888123
1000 0.332593262195587
10000 0.333381623029709
100000 0.340979009866714
};
\addlegendentry{$\sout=3000$}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/cava_10/vif_out_scales_sx_5000_epochs.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=1., xmax=1778279.41003892,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000,100000,1000000,10000000,100000000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{8}}\)
},
y grid style={darkgray176},
ylabel={vif},
ymin=0.17495726570487, ymax=0.373408968001604,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
10 0.221659243106842
100 0.187403857707977
1000 0.183977797627449
10000 0.184224650263786
100000 0.187441870570183
1000000 0.19004400074482
};
\addlegendentry{$\sout=30$}
\addplot [semithick, darkorange25512714]
table {%
10 0.306700170040131
100 0.226772040128708
1000 0.208392858505249
10000 0.207569792866707
100000 0.22047783434391
1000000 0.216040134429932
};
\addlegendentry{$\sout=100$}
\addplot [semithick, forestgreen4416044]
table {%
1 0.264978796243668
3 0.323644071817398
10 0.347332894802094
30 0.320815414190292
100 0.307585656642914
1000 0.299101978540421
10000 0.303500175476074
100000 0.295369565486908
1000000 0.308067739009857
};
\addlegendentry{$\sout=300$}
\addplot [semithick, crimson2143940]
table {%
1 0.245591461658478
3 0.321874469518661
10 0.362707942724228
30 0.345058768987656
100 0.330695331096649
1000 0.329155653715134
10000 0.329555660486221
100000 0.327009797096252
1000000 0.331350296735764
};
\addlegendentry{$\sout=1000$}
\addplot [semithick, mediumpurple148103189]
table {%
1 0.217094451189041
3 0.315077513456345
10 0.34495085477829
30 0.336706072092056
100 0.307657599449158
1000 0.319160789251328
10000 0.323832511901855
100000 0.327453553676605
1000000 0.317867159843445
};
\addlegendentry{$\sout=3000$}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/phantom/phantom_mse_out_scales_sx.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=0.501187233627272, xmax=1995262.31496888,
xmode=log,
ymode=log,
xtick style={color=black},
xticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{8}}\)
},
y grid style={darkgray176},
ylabel={mse},
ymin=-10.7362371921539, ymax=328.96076169014,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
1 15.505108833313
10 20.730785369873
100 15.7576112747192
1000 15.7941284179688
10000 15.8665714263916
100000 15.8681640625
1000000 15.801929473877
};
\addlegendentry{out scale = 10.0}
\addplot [semithick, darkorange25512714]
table {%
1 11.7098712921143
10 20.1888465881348
100 15.3309469223022
1000 15.5465278625488
10000 15.4999647140503
100000 13.2218580245972
1000000 5.25379991531372
};
\addlegendentry{out scale = 30.0}
\addplot [semithick, forestgreen4416044]
table {%
1 35.8871917724609
10 30.286003112793
100 4.87907600402832
1000 4.85523700714111
10000 4.70453548431396
100000 27.0151386260986
1000000 23.2766304016113
};
\addlegendentry{out scale = 100.0}
\addplot [semithick, crimson2143940]
table {%
1 73.7708969116211
10 313.519989013672
100 227.231704711914
1000 78.6054458618164
10000 138.940017700195
100000 150.353698730469
1000000 121.127975463867
};
\addlegendentry{out scale = 300.0}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/subsampled/phantom/phantom_vif_out_scales_sx.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={sx},
xmin=0.501187233627272, xmax=1995262.31496888,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000,100000,1000000,10000000,100000000},
xticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{8}}\)
},
y grid style={darkgray176},
ylabel={vif},
ymin=0.0265412444248796, ymax=0.184093378297985,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
1 0.0765930190682411
10 0.0847249701619148
100 0.0537870787084103
1000 0.0496247373521328
10000 0.0498258210718632
100000 0.0443177334964275
1000000 0.0467534922063351
};
\addlegendentry{out scale = 10.0}
\addplot [semithick, darkorange25512714]
table {%
1 0.0884810760617256
10 0.0987952575087547
100 0.0960623621940613
1000 0.0757236033678055
10000 0.0668014883995056
100000 0.132015556097031
1000000 0.167857438325882
};
\addlegendentry{out scale = 30.0}
\addplot [semithick, forestgreen4416044]
table {%
1 0.0869218483567238
10 0.105472892522812
100 0.175221472978592
1000 0.174196287989616
10000 0.176931917667389
100000 0.0658250749111176
1000000 0.0714748501777649
};
\addlegendentry{out scale = 100.0}
\addplot [semithick, crimson2143940]
table {%
1 0.0783279091119766
10 0.0377719476819038
100 0.0341513939201832
1000 0.0501875057816505
10000 0.0391492731869221
100000 0.0341914892196655
1000000 0.0337027050554752
};
\addlegendentry{out scale = 300.0}
\end{axis}

\end{tikzpicture}


==> figures/kfmlp/test.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.97)},
  anchor=north east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
width=\linewidth,
height=5cm,
x grid style={darkgray176},
xlabel={layer width},
xmajorgrids,
xmin=128, xmax=768,
xtick style={color=black},
xtick={128, 256, 384, 512, 768},
y grid style={darkgray176},
ylabel={maximum SER},
ymajorgrids,
ymin=16.9, ymax=17.2,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
    128 16.99
    256 17.08
    384 17.05
    512 17.04
    768 17.00
};


\end{axis}

\end{tikzpicture}


